Graph-Based Tests for Multivariate Covariate Balance Under Multi-Valued Treatments

We propose the use of non-parametric, graph-based tests to assess the distributional balance of covariates in observational studies with multi-valued treatments. Our tests utilize graph structures ranging from Hamiltonian paths that connect all of the data to nearest neighbor graphs that maximally separates data into pairs. We consider algorithms that form minimal distance graphs, such as optimal Hamiltonian paths or non-bipartite matching, or approximate alternatives, such as greedy Hamiltonian paths or greedy nearest neighbor graphs. Extensive simulation studies demonstrate that the proposed tests are able to detect the misspecification of matching models that other methods miss. Contrary to intuition, we also find that tests ran on well-formed approximate graphs do better in most cases than tests run on optimally formed graphs, and that a properly formed test on an approximate nearest neighbor graph performs best, on average. In a multi-valued treatment setting with breast cancer data, these graph-based tests can also detect imbalances otherwise missed by common matching diagnostics. We provide a new R package graphTest to implement these methods and reproduce our results.

==> latexmkrc.tex <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
	if (!($root_filename eq $_[0]))
	{
		system( "latexmk -cd -pdf \"$_[0]\"" );
	}
}

==> tables/applied_breast_mvt_test.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue May 25 11:10:50 2021
\begin{table*}[htb]
\centering
\begin{tabular}{lrrrr}
  \hline
 & k-Nearest Neighbor & Runs & Ranks & Crossmatch \\ 
  \hline
Baseline & $<1.1\times 10^{-16}$ & $<1.1\times 10^{-16}$ & $1 \times 10^{-09}$ & $<1.1\times 10^{-16}$ \\ 
  Cardinality matching (1st) & $2.2 \times 10^{-07}$ & $<1.1\times 10^{-16}$ & $4.3 \times 10^{-06}$ & $<1.1\times 10^{-16}$ \\ 
  Cardinality matching (2nd) & $7.8 \times 10^{-10}$ & $<1.1\times 10^{-16}$ & $3.2 \times 10^{-09}$ & $<1.1\times 10^{-16}$ \\ 
   \hline
\end{tabular}
\caption{Multisample tests applied to the matches from the cardinality matching methods. Baseline is the data before any adjustment and cardinality matching is done matching individuals in each treatment group to achieve group means within 0.05 standard deviations of the overall sample mean. (1st) is only matching first moments and (2nd) is matching first and all second moments.} 
\label{tab:applied_breast_mvt_test}
\end{table*}


==> tables/applied_breast_sample_size.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue May 25 11:10:50 2021
\begin{table*}[htb]
\centering
\begin{tabular}{rrrrrr}
  \hline
 & Treatment 1 & Treatment 2 & Treatment 3 & Treatment 4 & Treatment 5 \\ 
  \hline
Num. obs. & 636 & 1349 &  94 & 286 & 114 \\ 
   \hline
\end{tabular}
\caption{Sample size in each treatment group.} 
\label{tab:curated_breast_n}
\end{table*}


==> tables/applied_breast_uni_test.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue May 25 11:10:50 2021
\begin{table*}[htb]
\centering
\begin{tabular}{|l|ll|ll|ll|}
  \hline & \multicolumn{2}{C{2.7cm}|}{Baseline} & \multicolumn{2}{C{2.7cm}|}{Cardinality Matching (1st)} & \multicolumn{2}{C{2.7cm}|}{Cardinality Matching (2nd)} \\ \hline
Variable & Std. diff & p-value & Std. diff & p-value & Std. diff & p-value \\ 
  \hline
CASK & 0.81 & 0.00 & 0.04 & 0.54 & 0.05 & 0.98 \\ 
  CD47 & 0.45 & 0.00 & 0.04 & 0.93 & 0.04 & 0.72 \\ 
  COL6A1 & 0.46 & 0.00 & 0.04 & 0.45 & 0.06 & 0.22 \\ 
  COL6A2 & 0.56 & 0.00 & 0.05 & 0.28 & 0.05 & 0.26 \\ 
  CXADR & 0.27 & 0.00 & 0.04 & 0.87 & 0.05 & 0.60 \\ 
  DLC1 & 0.44 & 0.00 & 0.05 & 0.28 & 0.05 & 0.36 \\ 
  ER & 0.27 & 1.00 & 0.05 & 0.97 & 0.06 & 0.96 \\ 
  ETS2 & 0.74 & 0.00 & 0.04 & 0.33 & 0.06 & 0.18 \\ 
  FN1 & 0.50 & 0.00 & 0.04 & 0.44 & 0.04 & 0.46 \\ 
  GATA3 & 0.30 & 0.00 & 0.05 & 0.36 & 0.06 & 0.28 \\ 
  IGF1R & 0.41 & 0.00 & 0.03 & 0.62 & 0.04 & 0.35 \\ 
  IL6ST & 0.32 & 0.00 & 0.05 & 0.87 & 0.05 & 0.74 \\ 
  IRS2 & 0.52 & 0.00 & 0.05 & 0.67 & 0.05 & 0.47 \\ 
  LPP & 0.69 & 0.00 & 0.02 & 0.45 & 0.01 & 0.51 \\ 
  MBNL2 & 0.58 & 0.00 & 0.04 & 0.93 & 0.05 & 0.62 \\ 
  MYO10 & 0.47 & 0.00 & 0.04 & 0.36 & 0.05 & 0.87 \\ 
  NUDT4 & 0.40 & 0.00 & 0.05 & 0.34 & 0.05 & 0.52 \\ 
  P4HA1 & 0.44 & 0.00 & 0.01 & 0.58 & 0.04 & 0.37 \\ 
  PDCD4 & 0.11 & 0.00 & 0.04 & 0.33 & 0.06 & 0.27 \\ 
  Postmenopausal & 0.14 & 1.00 & 0.07 & 1.00 & 0.07 & 1.00 \\ 
  QKI & 0.37 & 0.00 & 0.02 & 0.42 & 0.05 & 0.31 \\ 
  RBPMS & 0.47 & 0.00 & 0.03 & 0.51 & 0.04 & 0.25 \\ 
  RGS5 & 0.56 & 0.00 & 0.04 & 0.40 & 0.05 & 0.98 \\ 
  SCD & 0.42 & 0.00 & 0.01 & 0.72 & 0.02 & 0.72 \\ 
  SLC12A2 & 0.20 & 0.00 & 0.04 & 0.50 & 0.04 & 0.65 \\ 
  SNRPN & 0.22 & 0.00 & 0.04 & 0.38 & 0.05 & 0.64 \\ 
  SOD2 & 0.36 & 0.00 & 0.01 & 0.71 & 0.01 & 0.75 \\ 
  SYNCRIP & 0.63 & 0.00 & 0.03 & 0.42 & 0.01 & 0.52 \\ 
  TACC1 & 0.57 & 0.00 & 0.03 & 0.86 & 0.02 & 0.79 \\ 
  TACC2 & 0.40 & 0.00 & 0.04 & 0.98 & 0.05 & 0.36 \\ 
  TFRC & 0.34 & 0.00 & 0.03 & 0.65 & 0.04 & 0.55 \\ 
  TMPO & 0.50 & 0.00 & 0.02 & 0.84 & 0.06 & 0.95 \\ 
   \hline
\end{tabular}
\caption{Univariate tests and absolute standardized mean differences applied to the matches/weights of various methods. Baseline is the data before any adjustment, and cardinality matching is done matching individuals in each treatment group to achieve group means within 0.05 standard deviations of the overall sample mean. (1st) is only matching first moments and (2nd) is matching first and all second moments.} 
\label{tab:applied_breast_uni_test}
\end{table*}

